Constructions for the optimal pebbling of grids

In [C. Xue, C. Yerger: Optimal Pebbling on Grids, Graphs and Combinatorics] the authors conjecture that if every vertex of an infinite square grid is reachable from a pebble distribution, then the covering ratio of this distribution is at most $3.25$. First we present such a distribution with covering ratio $3.5$, disproving the conjecture. The authors in the above paper also claim to prove that the covering ratio of any pebble distribution is at most $6.75$. The proof contains some errors. We present a few interesting pebble distributions that this proof does not seem to cover and highlight some other difficulties of this topic.

==> tikzstyles.tex <==

\tikzset{pebble/.style={shape          = circle,
                                 ball color     = blue,
                                 text           = white,
                                 inner sep      = 2pt,
                                 outer sep      = 0pt,}};
\tikzset{pebble2/.style={shape          = circle,
                                 ball color     = violet!50,
                                 text           = red,
                                 inner sep      = 2pt,
                                 outer sep      = 0pt,}};
\tikzset{tipus/.style={shape          = rectangle,
                                % ball color     = violet!10,
                                fill = white,
                                 text           = black,
                                 inner sep      = 0pt,
                                 outer sep      = 0pt,}};
\tikzset{csucs/.style={ circle,
                                % ball color     = violet!10,
                                fill = white,
                                % text           = black,
                                 inner sep      = 0pt,
                                 outer sep      = 0pt,
																}};
 \tikzset{szaggatott/.style={ultra thick, dashed}};
\tikzstyle{every path} = [>=stealth];
\tikzset{koord/.style={draw}};
\tikzstyle{nyil} = [>=latex,very thick,->];
